Differentiable Quantum Programming with Unbounded Loops

The emergence of variational quantum applications has led to the development of automatic differentiation techniques in quantum computing. Recently, Zhu et al. (PLDI 2020) have formulated differentiable quantum programming with bounded loops, providing a framework for scalable gradient calculation by quantum means for training quantum variational applications. However, promising parameterized quantum applications, e.g., quantum walk and unitary implementation, cannot be trained in the existing framework due to the natural involvement of unbounded loops. To fill in the gap, we provide the first differentiable quantum programming framework with unbounded loops, including a newly designed differentiation rule, code transformation, and their correctness proof. Technically, we introduce a randomized estimator for derivatives to deal with the infinite sum in the differentiation of unbounded loops, whose applicability in classical and probabilistic programming is also discussed. We implement our framework with Python and Q#, and demonstrate a reasonable sample efficiency. Through extensive case studies, we showcase an exciting application of our framework in automatically identifying close-to-optimal parameters for several parameterized quantum applications.

==> related_works.tex <==
\section{Related Works}\label{sec:related_works}
{
\subsubsection{Differentiation Rules of Quantum Circuits.}
There is a rich literature on differentiation rules of quantum circuits~\cite{schuld2019evaluating,PhysRevLett.118.150503,mitarai2018quantum,Banchi2021measuringanalytic,vidal2018calculus,wierichs2021general,izmaylov2021analytic,kyriienko2021generalized}.
These researches focus on how to use quantum hardware to derive the derivative of the expectation function of a parametrized quantum circuit.
For Pauli rotations $U(\theta) = e^{-i\theta \Delta/2}, \Delta=X,Y,Z$ in a PQC, \citet{PhysRevLett.118.150503} and \citet{mitarai2018quantum} first proposed a formula that only need to run the same PQC twice with different parameters to find the derivative.
Then, \citet{schuld2019evaluating} named this formula the ``parameter-shift rule'' and expanded it to a general case of $U(\theta) = e^{-i\theta H}$ with Hamiltonian $H$ having at most two distinct eigenvalues.
This parameter-shift rule has been adopted in many works~\cite{bergholm2018pennylane, broughton2020tensorflow, Zhu2020Differentiable,luo2020yao,kottmann2021tequila}.
Recently, independent developments of variants of the parameter-shift rules (general parameter-shift rules)~\cite{kyriienko2021generalized,izmaylov2021analytic,wierichs2021general} were proposed for general Hamiltonian $H$.
Their works can be traced back to an observation that the expectation function of a PQC with a single parameter is a finite Fourier series~\cite{vidal2018calculus}.
Moreover, for $U(\theta) = e^{-i(V+\theta H)}$, \citet{Banchi2021measuringanalytic} proposed the ``stochastic parameter-shift rule'' by means of an operator integral identity.

We propose a newly designed differentiation rule, the commutator-form rule, that is applicable to $e^{-i\theta H}$ for general $H$. 
This rule is based on a very different technique and has a simple form compared to general parameter-shift rules.

\subsubsection{Automatic Differentiation of Quantum Programs.}
Most existing automatic differentiation techniques in quantum computing~\cite{bergholm2018pennylane,luo2020yao,di2022quantum,kottmann2021tequila,nguyen2022qsun,broughton2020tensorflow} work with simple languages describing quantum circuits without any control flow, which follow directly from the aforementioned rules of quantum circuits. 
Note that some of them, e.g., \texttt{Yao.jl}~\cite{luo2020yao}, also apply classical automatic differentiation to classical programs that simulate parameterized quantum circuits, which is unfortunately not scalable for real quantum applications.  

The only exception and also the closest work to ours is \cite{Zhu2020Differentiable}, which proposed differentiable quantum programming with bounded loops beyond quantum circuits. 
Although the syntax in~\cite{Zhu2020Differentiable} supports general parameterized gates, 
its code transformation only supports Pauli rotation gates based on a variant of the parameter-shift rule.
To handle AD of bounded quantum loops, \citet{Zhu2020Differentiable} used a finite collection of quantum programs and added up their outputs for the derivative.
One cannot extend this approach to a collection of unbounded sizes like  unbounded loops in this paper.
Instead, this paper creates a random variable over an infinite domain to estimate the derivative, whose distribution must satisfy \ref{condition} to make the sampling estimation converge (correctness) and well-bounded for practical use (feasibility).
The correctness and feasibility of this paper to deal with infinite summation caused by unbounded loops is the main difficulty, which \citet{Zhu2020Differentiable} didn't encounter.
Moreover, the efficiency of this paper is comparable to~\cite{Zhu2020Differentiable} in the bounded-loop setting.
Thus, this paper strictly improves the AD technique in \cite{Zhu2020Differentiable}.
}
